Hallucination Detection and Hallucination Mitigation: An Investigation

Large language models (LLMs), including ChatGPT, Bard, and Llama, have achieved remarkable successes over the last two years in a range of different applications. In spite of these successes, there exist concerns that limit the wide application of LLMs. A key problem is the problem of hallucination. Hallucination refers to the fact that in addition to correct responses, LLMs can also generate seemingly correct but factually incorrect responses. This report aims to present a comprehensive review of the current literature on both hallucination detection and hallucination mitigation. We hope that this report can serve as a good reference for both engineers and researchers who are interested in LLMs and applying them to real world tasks.

==> reprodocued_results.tex <==

\section{Reproduced Results}
\label{sec: reproduce}
We have obtained some reproduced results for the aforementioned hallucination detection and mitigation methods. In this section, we will briefly show these results. 

\subsection{Reproduced results on detection}
Table~\ref{tab:hades_reproduced} shows reproduced results on Hades~\cite{liu2022token} detectors. We reproduced the results of Hades under the offline setting, i.e., the detector takes all tokens except the target token as the input, while predicting the hallucination label of the target token. We ran the code base of Hades and train the models from scratch. In Table~\ref{tab:hades_reproduced}, various metrics are reported for both the original results and the reproduced results. Most of the reproduced results align well with the original paper. However, due to the lack of specified hyper-parameters from the paper, there are some differences between the results. 

\begin{table}[!htbp]
\centering
\caption{Reproduced results for Hades~\cite{liu2022token} detectors. Results are reported in the format of original/reproduced. $\uparrow$ indicates higher the better, while $\downarrow$ indicates lower the better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|ccc|ccc}
\textbf{Reproduced} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Not Hallucination} & \multicolumn{3}{c}{Hallucination} \\ \hline
\textbf{Offline} & \multicolumn{1}{l|}{Acc~$\uparrow$} & \multicolumn{1}{l|}{G-Mean~$\uparrow$} & \multicolumn{1}{l|}{BSS~$\downarrow$} & \multicolumn{1}{l|}{AUC~$\uparrow$} & \multicolumn{1}{l|}{P~$\uparrow$} & \multicolumn{1}{l|}{R~$\uparrow$} & \multicolumn{1}{l|}{F1~$\uparrow$} & \multicolumn{1}{l|}{P~$\uparrow$} & \multicolumn{1}{l|}{R~$\uparrow$} & \multicolumn{1}{l}{F1~$\uparrow$} \\ \hline
LR & 63/62.25 & 63.02/60.77 & NA & NA & \multicolumn{1}{c|}{61.35/62.35} & \multicolumn{1}{c|}{64.89/72.08} & 63.07/66.86 & \multicolumn{1}{c|}{64.74/62.1} & \multicolumn{1}{c|}{61.21/51.23} & 62.92/50.33 \\
SVM & 62.2/63.67 & 61.2/61.5 & NA & NA & \multicolumn{1}{c|}{58.72/62.89} & \multicolumn{1}{c|}{75.35/76.18} & 66.01/68.9 & \multicolumn{1}{c|}{68/65.05} & \multicolumn{1}{c|}{49.7/49.65} & 57.43/56.31 \\
Bert\_Hades & 71/71.92 & 70.42/71.95 & 20.94/19.06 & 75.76/78.63 & \multicolumn{1}{c|}{73.39/74.46} & \multicolumn{1}{c|}{63.44/71.29} & 68.06/72.85 & \multicolumn{1}{c|}{69.26/69.31} & \multicolumn{1}{c|}{78.17/70.67} & 73.44/70.92 \\
RoBERTa\_Hades & 69.04/72.83 & 68.03/70.94 & 19.44/18.78 & 76.47/78.72 & \multicolumn{1}{c|}{70.08/74.06} & \multicolumn{1}{c|}{68.03/74.76} & 69.04/74.41 & \multicolumn{1}{c|}{67.33/71.43} & \multicolumn{1}{c|}{68.03/70.67} & 68.35/71.05 \\
XLNet\_Hades & 70.5/72.33 & 68.6/71.39 & 19.5/18.79 & 78.19/78.93 & \multicolumn{1}{c|}{70.05/71.15} & \multicolumn{1}{c|}{79.33/80.13} & 74.45/75.37 & \multicolumn{1}{c|}{74.70/74.07} & \multicolumn{1}{c|}{64.27/63.60} & 69.09/68.44
\end{tabular}%
}
\label{tab:hades_reproduced}
\end{table}

Table~\ref{tab:selfcheckgpt_reproduced}, shows reproduced results on SelfCheckGPT~\cite{manakul2023selfcheckgpt} detectors. We reproduced the results of SelfCheckGPT under the three different tasks as outlined in the original paper. Recall there are three labels in the dataset created by the authors: minor-inaccurate, major-inaccurate and accurate. In detecting non-fact sentences, both major-inaccurate labels and minor-inaccurate labels are grouped together into the non-factual class, while the factual class refers to accurate sentences. In addition, the authors also consider a more challenging task of detecting major-inaccurate sentences in passages that are not total hallucination passages, which is referred to as non-factual$^*$. SelfCheckGPT comes as a python package. We coded the experiment pipeline using the package and report the AUC-PR scores in Table~\ref{tab:selfcheckgpt_reproduced}. The results are extremely consistent with the original paper. 

\begin{table}[!htbp]
\centering
\caption{Reproduced results for SelfCheckGPT~\cite{manakul2023selfcheckgpt} detectors. Results are reported in the format of original/reproduced. Higher the better.}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{l|lll}
Reproduced & \multicolumn{3}{c}{Sentence-level (AUC-PR)} \\ \hline
SelfCheckGPT & \multicolumn{1}{l|}{Nonfact} & \multicolumn{1}{l|}{Nonfact*} & Factual \\ \hline
w/ Bertscore & \multicolumn{1}{l|}{81.96/81.96} & \multicolumn{1}{l|}{45.97/45.96} & 44.21/44.23 \\
w/ QA & \multicolumn{1}{l|}{84.21/84.26} & \multicolumn{1}{l|}{40.06/40.06} & 48.10/48.14 \\
w/ Unigram & \multicolumn{1}{l|}{85.64/85.63} & \multicolumn{1}{l|}{41.05/41.04} & 58.43/58.47
\end{tabular}%
}
\label{tab:selfcheckgpt_reproduced}
\end{table}


In Table~\ref{tab:enfa_reproduced}, shows the reproduced results on EnFa~\cite{cao-etal-2022-hallucinated} detectors. We ran the code base of EnFa and train the models from scratch. In Table~\ref{tab:enfa_reproduced}, we report the reproduced accuracy as well as F1 score on both hallucination and factual classes. The reproduced results are fairly consistent with the original paper. 

\begin{table}[!htbp]
\centering
\caption{Reproduced results for EnFa~\cite{cao-etal-2022-hallucinated} detectors. Higher the better.}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{l|ll|ll}
EnFa & \multicolumn{2}{l|}{Hallucination} & \multicolumn{2}{l}{Facturality} \\ \hline
 & \multicolumn{1}{l|}{Acc} & F1 & \multicolumn{1}{l|}{Acc} & F1 \\ \hline
Reproduced & \multicolumn{1}{l|}{91.5} & 90.2 & \multicolumn{1}{l|}{91.26} & 83.11 \\
original & \multicolumn{1}{l|}{93.09} & 91.01 & \multicolumn{1}{l|}{90.95} & 81.82
\end{tabular}%
}
\label{tab:enfa_reproduced}
\end{table}


Table~\ref{tab:cnsg_reproduced} shows the reproduced results on CNSG~\cite{zhou2021detecting} detectors. The training data is not provided in the code base. Therefore, the reproduced results were obtained by directly evaluating the model that the authors provide. 
In Table~\ref{tab:cnsg_reproduced}, we report the reproduced F1 score on the summaries obtained by various abstractive summarization systems: PtGen~\cite{see2017get}, TConvS2S~\cite{narayan-etal-2018-dont}, TranS2S~\cite{vaswani2017attention} and BERTS2S~\cite{rothe2020leveraging}. The reproduced results are fairly consistent with the original paper. 

\begin{table}[!htbp]
\caption{Reproduced results for CNSG~\cite{zhou2021detecting} detectors. Results are reported in the format of original/reproduced. Higher the better.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llll}
F1 & PtGen & TConvS2S & TransS2S & BERTS2S \\ \hline
w/o refeence & 63.12/63.66 & 65.36/65.94 & 60.99/61.70 & 55.57/55.45 \\
w/o reference + synonym & 64.21/64.72 & 69.11/69.37 & 63.81/63.88 & 56.48/56.49 \\
w/ reference & 63.19/63.89 & 65.89/66.28 & 62.10/62.24 & 55.88./55.88
\end{tabular}%
}
\label{tab:cnsg_reproduced}
\end{table}


\subsection{Reproduced results on mitigation}
%
In Table~\ref{tab:nph_mitigation}, we present the results obtained from reproducing using Neural Path Hunter (NPH) model~\cite{dziri2021neural} to generate refined responses.
%
We trained the NPH model on the OpenDialKG~\cite{moon2019opendialkg}, adhering to the same split setting as in paper ( 80\%/10\%/10\ resulting in 61778 train, 7933 valid and 7719 test, respectively). 
%
For the training, we had a preliminary test using the GPT-2 as the base model, maintaining the same default model and hyperparameters as in the Github open-source code \footnote{https://github.com/nouhadziri/Neural-Path-Hunter}, except for a smaller batch size (6) (due to the memory limit on a RTX 3080), and a larger number of training epochs (12).
%


\begin{table}[!htbp]
\centering
\caption{Reproduced results for NPH~\cite{dziri2021neural} model for hallucination mitigation.}
\resizebox{0.27\textwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Model & FeQA & BLEU \\ \midrule
GPT2 & 13.2 & 9.06 \\
GPT2 + NPH & 14.0 & 9.5 \\ \midrule
\end{tabular}
}
\label{tab:nph_mitigation}
\end{table}

%
As a preliminary result, we directly ran the source code under its default setup, which uses the Hugging Face \textit{GPT2} model \footnote{https://huggingface.co/gpt2}. In Table~\ref{tab:nph_mitigation}, we show the reproduced result. Similar to the original paper, we evaluate the FeQa~\cite{durmus-etal-2020-feqa} and the BLEU~\cite{papineni2002bleu} metrics of the generated responses from GPT2 directly (GPT2) and with the NPH refinement (GPT2+NPH). We observe that NPH does help improving the performances on these two metrics. 

Note in the original paper, the base model is selected to be GPT2-KG~\cite{radford2019language}, which is a pre-trained GPT2 model that has been fine-tuned on a dialogue corpus. Out next step of reproduction is to train and evaluate NPH on GPT2-KG and compare the results with the original paper.

% The reproduced results show some difference compared to the results in Table. \ref{tab:nph_mitigation_original}, which are potentially be due to differences in the model and training configurations.
% %
% In the original paper, the base model utilized is GPT-KG~\cite{radford2019language}, a pre-trained GPT-2 model that has been fine-tuned on a dialogue corpus.
% %
% We used the Hugging Face \textit{gpt2} model \footnote{https://huggingface.co/gpt2}, default in the source code.
% %
% Despite the difference, our results demonstrate that the application of NPH refinement leads to an improvement in FeQA scores same as in the original paper.
% %


% \begin{table}[!htbp]
% \centering
% \caption{Original results for NPH~\cite{dziri2021neural} model for hallucination mitigation.}
% \resizebox{0.3\textwidth}{!}{%
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Model & FeQA & BLEU \\ \midrule
% GPT2-KG & 26.54 & 11.79 \\
% GPT2-KG  + NPH & 28.98 & 11.29 \\ \midrule
% \end{tabular}
% }
% \label{tab:nph_mitigation_original}
% \end{table}




% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc}
% RHO &  &  & \multicolumn{2}{c}{QuestEval} \\ \hline
% Methods & \multicolumn{1}{c|}{RogueL} & Bleu4 & \multicolumn{1}{c|}{RF} & RD \\ \hline
% Local & \multicolumn{1}{c|}{39.96/39.38} & 19.89/19.47 & \multicolumn{1}{c|}{44.37/43} & 48.91/48.32 \\
% Global & \multicolumn{1}{c|}{39.54/39.46} & 20.7719.59 & \multicolumn{1}{c|}{43.84/42.54} & 48.41/47.76 \\
% Global+local & \multicolumn{1}{c|}{39.51/39.4} & 20.63/19.44 & \multicolumn{1}{c|}{46.03/45.14} & 50.35/49.78 \\
% Full & \multicolumn{1}{c|}{38.45/38.12} & 19.11/19.02 & \multicolumn{1}{c|}{46.41/45.89} & 50.58/49.96
% \end{tabular}%
% }
% \caption{Reproduced results for RHO~\cite{ji2023rho} handler. Results are reported in the format of original/reproduced. Higher the better.}
% \label{tab:rho_reproduced}
% \end{table}

